Low-Rank Adaptation of Geospatial Foundation Models for Wildfire Mapping Using Sentinel-2 Data

Wildfire burned-area mapping is essential for damage assessment, emissions modeling, and understanding fire-climate interactions across diverse ecological regions. Recent geospatial foundation models provide strong general-purpose representations for satellite imagery, yet there is still no clear understanding of how to efficiently adapt these models for downstream Earth observation tasks, particularly under geographic and temporal domain shift. This study evaluates three state-of-the-art Geospatial Foundation Models (GFMs) - Terramind, DINOv3, and Prithvi-v2 - for burned-area mapping across the United States and Canada using Sentinel-2 data. Leveraging 3,820 wildfire events from 2017-2023, we conduct spatial and temporal generalization tests across diverse biomes. We systematically compare full fine-tuning, decoder-only fine-tuning, and Low-Rank Adaptation (LoRA) for adapting each model. Across all experiments, LoRA provides the strongest cross-domain generalization while updating less than 1% of parameters, demonstrating a favorable trade-off between accuracy and efficiency. Prithvi-v2 with LoRA achieves the highest overall accuracy and the largest improvement compared to full fine-tuning. These findings indicate that geospatial foundation models, when adapted using lightweight parameter-efficient methods such as LoRA, offer a robust and scalable solution for large-scale burned-area mapping. Code is available at https://github.com/alishibli97/wildfire-lora-gfm.

==> sections/1_introduction_before.tex <==
\section{Introduction}

The emergence of large-scale geospatial foundation models (GFMs) such as 
Prithvi, Clay, TerraMind, and others 
has fundamentally improved downstream remote-sensing performance 
\cite{ssl4eo,prithvi,clay,terramind}. Trained on multimillion-image datasets 
using self-supervision, GFMs provide general-purpose representations that 
transfer effectively to tasks such as land cover mapping, flood segmentation, 
disaster response, and environmental monitoring.

However, GFMs are trained differently: they vary in input modalities (RGB, 
multispectral, SAR), pretraining datasets, tokenization schemes, and 
architectures. Recent studies show complementary strengths across different GFMs 
\cite{peft_geofm,deflect,csmoe}, yet typical practice restricts users to 
selecting only one.

This leads to a key gap in the literature:
\begin{quote}
\emph{No prior work investigates whether multiple GFMs can be fused cheaply to 
achieve representations strictly better than each model alone.}
\end{quote}

Full multi-GFM ensembling is infeasible: modern GFMs contain hundreds of 
millions of parameters. Fine-tuning several simultaneously multiplies compute, 
memory, and optimization instability. Parameter-efficient fine-tuning (PEFT) 
methods such as LoRA \cite{lora} provide a promising direction: they allow small 
rank-constrained updates on top of frozen backbones, reducing computational cost 
by 10--100$\times$.

\subsection{Contributions}

We propose the first parameter-efficient method for multi-GFM fusion:
\begin{itemize}
    \item We introduce LoRA adapters for each GFM, enabling task-specific 
          adaptation without modifying pretrained weights.
    \item We fuse multiple GFM embeddings through a shared lightweight decoder 
          that learns cross-model complementarities.
    \item We demonstrate improved segmentation accuracy over individual GFMs on 
          diverse datasets using less than 5\% of the parameters of full 
          fine-tuning.
    \item We analyze the complementary behaviour of GFMs and show that the fused 
          architecture consistently captures richer spatial structure.
\end{itemize}

